End-to-end Text-to-speech for Low-resource Languages by Cross-Lingual Transfer Learning

End-to-end text-to-speech (TTS) has shown great success on large quantities of paired text plus speech data. However, laborious data collection remains difficult for at least 95% of the languages over the world, which hinders the development of TTS in different languages. In this paper, we aim to build TTS systems for such low-resource (target) languages where only very limited paired data are available. We show such TTS can be effectively constructed by transferring knowledge from a high-resource (source) language. Since the model trained on source language cannot be directly applied to target language due to input space mismatch, we propose a method to learn a mapping between source and target linguistic symbols. Benefiting from this learned mapping, pronunciation information can be preserved throughout the transferring procedure. Preliminary experiments show that we only need around 15 minutes of paired data to obtain a relatively good TTS system. Furthermore, analytic studies demonstrated that the automatically discovered mapping correlate well with the phonetic expertise.

==> figs/cer_mcd.tex <==
\begin{figure}[h]
  \centering
  \includegraphics[width=.45\textwidth]{figs/cer_mcd.png}
  \caption{ASR recognition and MCD objective tests on Mandarin, German and French. For Mandarin and German, full training target data is 30 minutes, and for French, 15 minutes is used.}
  \label{fig:cer_mcd}
\end{figure}

==> tables/prep_hparam.tex <==
\begin{table}[h]
\caption{Speech recognition/synthesis setting}
  \label{tab:preprocessing}
  \centering
\begin{tabular}{l | l}
  Pre-emphasis & $0.97$  \\
  \hline
  Frame length & $50$ ms  \\
  \hline
  Frame shift & $12.5$ ms  \\
  \hline
  Window type & Hann    \\
  \hline
  Sample rate & $20$k (TTS) / $16$k (ASR) \\
  \hline
  Mel-spectrogram & $80$ \\
  \hline
  Linear-spectrogram & $1025$ \\
\end{tabular}
\end{table}

==> tables/preprocess_hparam.tex <==
\begin{table}[h]
\caption{Speech recognition/synthesis setting}
  \label{tab:preprocessing}
  \centering
\begin{tabular}{l | l}
  Pre-emphasis & $0.97$  \\
  \hline
  Frame length & $50$ ms  \\
  \hline
  Frame shift & $12.5$ ms  \\
  \hline
  Window type & Hann    \\
  \hline
  Sample rate & $20$k (TTS) / $16$k (ASR) \\
  \hline
  Mel-spectrogram & $80$ \\
  \hline
  Linear-spectrogram & $1025$ \\
\end{tabular}
\end{table}
